Beyond Silence: Bias Analysis through Loss and Asymmetric Approach in Audio Anti-Spoofing

Current trends in audio anti-spoofing detection research strive to improve models' ability to generalize across unseen attacks by learning to identify a variety of spoofing artifacts. This emphasis has primarily focused on the spoof class. Recently, several studies have noted that the distribution of silence differs between the two classes, which can serve as a shortcut. In this paper, we extend class-wise interpretations beyond silence. We employ loss analysis and asymmetric methodologies to move away from traditional attack-focused and result-oriented evaluations towards a deeper examination of model behaviors. Our investigations highlight the significant differences in training dynamics between the two classes, emphasizing the need for future research to focus on robust modeling of the bonafide class.

==> figures/loss_trend.tex <==
\begin{figure}
    %\floatsetup{heightadjust=all, valign=c}
    %\ffigbox{\begin{subfloatrow}[2]
        \ffigbox[\FBwidth]{\includegraphics[width=0.5\textwidth]{bona_loss.png}}
        {\caption{bonafide class loss} \label{fig:bona_loss}}
        %\hspace*{\dimexpr-\tabcolsep}
        \hspace{-1.5cm}
        \ffigbox[\FBwidth]{\includegraphics[width=0.5\textwidth]{spoof_loss.png}}
        {\caption{spoof class loss}\label{fig:spoof_loss}}
    %\end{subfloatrow}}
    {\caption{Training loss for each class during the training}\label{fig:loss_trend}}
\end{figure}

==> sections/0_abstract_prev.tex <==
Current trends in audio anti-spoofing detection research strive to improve models' ability to generalize across unseen attacks by learning to identify a variety of spoofing artifacts. This emphasis has primarily focused on the spoof class. 
However, recent efforts have begun to explore the distinctions between bonafide and spoof class, particularly through the lens of `silence'.
Our study expands upon class-wise interpretations beyond the silence. We utilize loss analysis and asymmetric methodologies to shift from traditional attack-centric and result-oriented evaluations toward a more in-depth exploration of model behaviors.
Our investigations reveal the significant differences in training dynamics between the two classes, underlining the necessity for future research to concentrate on the robust modeling of the bonafide class.

==> sections/legacy_related_works.tex <==
\iffalse
\section{Related works}
In this section, we will introduce the most relevant works to our research, the previous findings related to the data bias in audio anti-spoofing. %asymmetric architecture 
%generic approach for data bias analysis~\cite{}. The former is to understand the mainstream work in this domain, which also contradicts our findings in the end. The latter one is used as our analysis tool with some modification so that needs to be understood. 
There are comparably few works done with data bias in audio anti-spoofing while most of the research has been being eager to improve the numerical performance. 
In earlier works, the uneven distribution of waveform for each class has been raised as the main factor that influences their predictions~\cite{chettri2018deeper} - genuine signals include more zero but the spoofed signals include less. It was investigated upon ASVspoof2017 dataset~\cite{} which covers physical attack, generated spoof speech with replay attack.
Later after the ASVspoof2019 data was published followed by the ASVspoof2017 dataset, similar findings were discovered in several works~\cite{lapidot2020effects, muller2021speech, zhang2023impact}.
In summary, \textit{silence}, the proportion of zero-valued in speech, is a main concern that induced the model to undesirably operate.
However, silence is hard to investigate deeply as it could be affected by both the type of source data and the data generation process.
Moreover, other data bias is barely covered other than silence in this domain although such direction of work is necessary to better understand the current models which helps to be developed further. 
\fi

==> tables/config_jee.tex <==
\begin{table}[!t] 
    \caption{Five experimental configurations using eight subsets of a dataset. O is the original (unintervened) configuration. All other four sets have one particular subset intervened.}
    \label{tab:config_jee}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c}
    \toprule
    Intervened phase & Configuration & Train set& Test set\\
         \hline
         - & \textbf{O} & $\mathcal{D}_\text{trn, bona} \cup \mathcal{D}_\text{trn,spf}$  & $\mathcal{D}_\text{test, bona} \cup \mathcal{D}_\text{test, spf}$  \\
         \toprule
         \multirow{2}{*}{Train} & \textbf{Tr\_B} & $\mathcal{D}^{\textbf{intervene}}_\text{trn, bona} \cup \mathcal{D}_\text{trn,spf}$  & $\mathcal{D}_\text{test, bona} \cup \mathcal{D}_\text{test, spf}$ \\
         %\cline{3-4}
         & \textbf{Tr\_S} & $\mathcal{D}_\text{trn, bona} \cup \mathcal{D}^{\textbf{intervene}}_\text{trn,spf}$  & $\mathcal{D}_\text{test, bona} \cup \mathcal{D}_\text{test, spf}$ \\
         \toprule
         \multirow{2}{*}{Test} & \textbf{Te\_B}  & $\mathcal{D}_\text{trn, bona} \cup \mathcal{D}_\text{trn,spf}$  & $\mathcal{D}^{\textbf{intervene}}_\text{test, bona} \cup \mathcal{D}_\text{test, spf}$\\
         %\cline{3-4}
         & \textbf{Te\_S}  & $\mathcal{D}_\text{trn, bona} \cup \mathcal{D}_\text{trn,spf}$  & $\mathcal{D}_\text{test, bona} \cup \mathcal{D}^{\textbf{intervene}}_\text{test, spf}$\\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/silence_trim.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
  \caption{Performance comparison in EER when the model \textbf{tested} on a asymmetric ways with silence trimming. Silence trimming is also exploited either train or test, and both. The bold type indicates the case that spoof side intervention lower EER than the bonafide one.} 
  \centering
  \label{tab:silence_trim}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{l|l|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{System}} & \multicolumn{1}{c|}{\multirow{2}{*}{Silence   trimming}} & \multicolumn{3}{c|}{Mp3} & \multicolumn{3}{c|}{Noise} & \multicolumn{3}{c}{Loudness} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \textbf{Te\_S} & \textbf{Te\_B} & ratio & \textbf{Te\_S} & \textbf{Te\_B} & ratio & \textbf{Te\_S} & \textbf{Te\_B} & ratio \\
    \hline
    Original & - & 1.21 & 8.78 & 7.26 & 0.65 & 35.50 & 54.62 & 2.23 & 6.73 & 3.08 \\
    RawBoost & - & 1.62 & 3.96 & 2.44 & 1.06 & 13.27 & 12.52 & 1.52 & 2.38 & 1.57 \\ \hline
    Original & train & 28.36 & 39.32 & 1.39 & 47.09 & 28.14  & \textbf{0.60} & 27.44 &  47.28 & 1.72 \\
     & test & 20.07 & 37.7 & 1.88 & 8.27 & 59.04 & 7.14 & 13.92 & 40.83 & 2.93 \\
     & train\&test & 17.52 & 30.65 & 1.75 & 17.24 & 34.49 & 2.00 & 14.79 & 26.99 & 1.82 \\ \hline
    
    RawBoost & train & 40.65 & 48.47 & 1.19 &  66.93 & 31.14 & \textbf{0.47} &36.10 & 55.35 & 1.53\\
     & test & 29.5 & 30 & 1.02 & 30.74 & 26.85 & \textbf{0.87} & 21.82 & 37.05 & 1.70 \\
     & train\&test & 17.56 & 31.69 & 1.80 & 21.07 & 32.35 & 1.54 & 12.75 & 29.73 & 2.33 \\
    \bottomrule
    \end{tabular}
}
\end{table*}
